An Analysis on the Influence of Network Topologies on Local and Global Dynamics of Metapopulation Systems

Metapopulations are models of ecological systems, describing the interactions and the behavior of populations that live in fragmented habitats. In this paper, we present a model of metapopulations based on the multivolume simulation algorithm tau-DPP, a stochastic class of membrane systems, that we utilize to investigate the influence that different habitat topologies can have on the local and global dynamics of metapopulations. In particular, we focus our analysis on the migration rate of individuals among adjacent patches, and on their capability of colonizing the empty patches in the habitat. We compare the simulation results obtained for each habitat topology, and conclude the paper with some proposals for other research issues concerning metapopulations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{P. Milazzo and M.J. P\'erez Jim\'enez (Eds.): Applications of Membrane Computing,\\
Concurrency and Agent-based Modelling in Population Biology (AMCA-POP 2010)\\
EPTCS 33, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.33.1}{10.4204/EPTCS.33.1}}

